Multilevel weighted least squares polynomial approximation

Weighted least squares polynomial approximation uses random samples to determine projections of functions onto spaces of polynomials. It has been shown that, using an optimal distribution of sample locations, the number of samples required to achieve quasi-optimal approximation in a given polynomial subspace scales, up to a logarithmic factor, linearly in the dimension of this space. However, in many applications, the computation of samples includes a numerical discretization error. Thus, obtaining polynomial approximations with a single level method can become prohibitively expensive, as it requires a sufficiently large number of samples, each computed with a sufficiently small discretization error. As a solution to this problem, we propose a multilevel method that utilizes samples computed with different accuracies and is able to match the accuracy of single-level approximations with reduced computational cost. We derive complexity bounds under certain assumptions about polynomial approximability and sample work. Furthermore, we propose an adaptive algorithm for situations where such assumptions cannot be verified a priori. Finally, we provide an efficient algorithm for the sampling from optimal distributions and an analysis of computationally favorable alternative distributions. Numerical experiments underscore the practical applicability of our method.

==> content/MCMC.tex <==

%\Cref{pro:stability} shows that if the optimal densities $\optimaldensity_{l}$ associated to a sequence $(\vsp_l)_{l\in\N}$ of polynomial spaces converge to a limit $\optimaldensity_{\infty}$ in an appropriate sense, then we may use samples from $\optimaldensity_{\infty}\measure$ for all $l$ without changing the asymptotic behavior of the approximation error. Next, we study conditions under which such a limit exists. Furthermore, even when no limit exists, we derive upper and lower bounds on $\optimaldensity$ that are independent of the polynomial space. A lower bound on $\optimaldensity$ allows to get rid of the weight $\sqrt{\weight(\psmi)}=1/\sqrt{\optimaldensity}$ in the definition of $e_{\vsp,\infty}(\rs)$ in \Cref{eq:bestlinf}, thus making it easier to verify bounds on this quantity in practice. An upper bound on $\optimaldensity$ allows for the application of Markov Chain methods to obtain samples from $\optimaldensity\measure$.

%\input{./content/optimaldensities}




%To extend \Cref{alg:MCMC} to measures on $\R^d$, the arcsine distribution $\arcsine$ needs to be replaced by one supported on all of $\R$. For example, it is known that if $\measure$ is Gaussian, then the sampling measure $\density_m\measure$ concentrates on an interval of size $[-a_m,a_m]$ with $a_m\approx m^{1/2}$ \cite{}.

==> content/optimaldensities.tex <==
Recall from \Cref{eq:optimalmeasure} that the optimal density associated to a polynomial space $\vsp$ and a measure $\measure$ is the mean square function of a $L^2(\measure)$-orthonormal basis $(L_j)_{j=1}^{\dvsp}$ of $\vsp$,
\begin{equation*}
\optimaldensity(\psmi):=\frac{1}{\dvsp}\sum_{j=1}^{\dvsp}|L_j(\psmi)|^2.
\end{equation*}
 The theory of orthogonal univariate polynomials shows that for $\domPS:=[0,1]$ the optimal sampling measures $\samplingmeasure_{k}=\optimaldensity_{k}\measure$ associated to spaces $\polka([0,1])$ of polynomials of degree less than or equal to $k$ converge to the arcsine distribution with Lebesgue density
\begin{equation}
\label{eq:arcsine}
\arcsine_{1}(\psmi)=\frac{1}{\pi \sqrt{\psmi(1-\psmi)}}, \quad\psmi\in[0,1]
\end{equation}
as $k\to\infty$, under rather permissive assumptions on $\measure$ \cite{}.
In other words, the density $\optimaldensity$ converges to $\frac{d\lambda}{d\measure}\arcsine_{1}$, where $\lambda$ is the Lebesgue measure and $\frac{d\lambda}{d\measure}$ the Radon-Nikodym derivative. 

By \Cref{pro:stability} we may thus use samples from $\arcsine_{1}\lambda$ for any choice of $\measure$ and any $k\in\N$ without changing the asymptotic behavior of the approximation error in \Cref{thm:dpls}. Conveniently, samples from $\arcsine_{1}$ can be computed as $\sin(X)$, for a uniform random variable $X$ on $[-\pi/2,\pi/2]$.

In the multivariate setting, if the space of polynomials $\vsp$ under consideration is a tensor product space $\vsp=\bigotimes_{j=1}^{d}\polka([0,1])$ and if $\measure$ is a product measure, then the associated optimal sampling measure $\samplingmeasure=\optimaldensity\measure$ is the product of the univariate ones and converges to the $d$-fold tensor product of the arcsine distribution,
 \begin{equation*}
 \arcsine_{d}(\psmi):=\prod_{j=1}^{d}\frac{1}{\pi\sqrt{\psmi(1-\psmi)}},\quad \psmi\in[0,1]^d
 \end{equation*}
 as $k\to\infty$. However, this does not hold in general. For example, for the space $\vsp_{k,\psmi_1}\oplus \vsp_{k,\psmi_2}=\vspan\{1,\psmi_1,\psmi_2,\psmi_1^2,\psmi_2^2,\dots,\psmi_1^k,\psmi_2^k\}$ of polynomials on $[0,1]^2$ equipped with the Lebesgue measure we have
\begin{equation*}
\begin{split}
\optimaldensity_k(\psmi)&=\frac{1}{2k}\left(\sum_{j=1}^{k}|L_j(\psmi_1)|^2+\sum_{j=1}^{k}|L_j(\psmi_2)|^2\right)\\
&\to \frac{1}{2\pi\sqrt{\psmi_1(1-\psmi_1)}}+\frac{1}{2\pi\sqrt{\psmi_2(1-\psmi_2)}}
\end{split}
\end{equation*}
as $k\to\infty$. The limit density in this case is still bounded by the $d$-dimensional arcsine distribution, which is a special case of the following proposition.
%This shows that we cannot simply replace the optimal measure $\density_{*}\measure$ by the $d$-fold tensor product of the arcsine distribution in \Cref{eq:arcsine}.
 %For example, if  To the best of our knowledge, little is known about the behavior of $\samplingmeasure_{\vsp}=\density_{\vsp}\measure$ for general spaces $\vsp$ and measures $\measure$. In any case, we do 


